Energy-Calibrated VAE with Test Time Free Lunch

In this paper, we propose a novel generative model that utilizes a conditional Energy-Based Model (EBM) for enhancing Variational Autoencoder (VAE), termed Energy-Calibrated VAE (EC-VAE). Specifically, VAEs often suffer from blurry generated samples due to the lack of a tailored training on the samples generated in the generative direction. On the other hand, EBMs can generate high-quality samples but require expensive Markov Chain Monte Carlo (MCMC) sampling. To address these issues, we introduce a conditional EBM for calibrating the generative direction of VAE during training, without requiring it for the generation at test time. In particular, we train EC-VAE upon both the input data and the calibrated samples with adaptive weight to enhance efficacy while avoiding MCMC sampling at test time. Furthermore, we extend the calibration idea of EC-VAE to variational learning and normalizing flows, and apply EC-VAE to an additional application of zero-shot image restoration via neural transport prior and range-null theory. We evaluate the proposed method with two applications, including image generation and zero-shot image restoration, and the experimental results show that our method achieves competitive performance over single-step non-adversarial generation. Our code is available at https://github.com/DJ-LYH/EC-VAE.

==> Tables/tab_celeba64_256.tex <==
\begin{table}
\vspace{-2mm}
\centering
\begin{tabular}{cc}
    \begin{minipage}[t]{1.5in}
                \caption{\small Generative performance on CelebA.}
               \label{tab:celeba64} 
               \centering
        \scalebox{0.8}{
\begin{tabular}{@{}lc@{}}
\hline
\toprule
      \textbf{Model} & \textbf{FID$\downarrow$}\\
      \midrule
      NCSNv2~\cite{song2020improved} & 26.86 \\
      \midrule
      COCO-GAN~\cite{lin2019coco} & \textbf{4.0} \\
      QA-GAN~\cite{parimala2019quality} & 6.42 \\
      Divergence Triangle~\cite{han2020joint} & 24.7 \\
      % Flow CE~\cite{gao2020flow} & 12.21\\ At celeba 32, Not celeba 64
      \midrule
      \midrule
      VAEBM~\cite{vaebm} & 5.31\\
      NCP-VAE~\cite{nvp-vae} & 5.25 \\
      NVAE~\cite{vahdat2020NVAE} & 14.74\\
      \midrule
      \textbf{\shortname (Ours)} & \textbf{4.20} \\
\bottomrule
\hline
\end{tabular}
}
\end{minipage}

&
    \begin{minipage}[t]{1.5in}
        \caption{\small Generative performance on CelebA-HQ.} 
        \label{tab:celeba256}
        \centering
        \scalebox{0.8}{
\begin{tabular}{@{}lc@{}}
\hline
    \toprule
      \textbf{Model} & \textbf{FID$\downarrow$} \\
    \midrule
      ALAE~\cite{pidhorskyi2020adversarial} & 19.21\\
      DC-VAE~\cite{dcvae} & 15.81\\
      PGGAN~\cite{karras2017progressive} & \textbf{8.03}\\
      \midrule
    \midrule
      GLOW~\cite{kingma2018glow}&68.93\\
      \midrule
      VAEBM~\cite{vaebm}& 20.38\\
      NCP-VAE~\cite{nvp-vae} & 24.79 \\
      NVAE~\cite{vahdat2020NVAE} & 45.11\\
      \midrule
      \textbf{\shortname (Ours)} & \textbf{13.62} \\
\bottomrule
\hline
\end{tabular}
}
\end{minipage}
\end{tabular}
\vspace{-3mm}
\end{table}


==> Tables/tab_stl_imagnet.tex <==
\begin{table}
\vspace{-4mm}
\centering
\begin{tabular}{ccc}
    \begin{minipage}[t]{1.5in}
        \caption{\small Generative performance on STL-10.}
        \label{tab:stl} 
        \centering
        \scalebox{0.8}{
            \begin{tabular}{@{}lc@{}}
                \hline
                \toprule
                \textbf{Model} & \textbf{FID$\downarrow$} \\
                \midrule
                ProbGAN~\cite{he2019probgan}   & 46.7 \\
                SN-GAN~\cite{miyato2018spectral}    & 40.1  \\
                Improv. MMD GAN~\cite{wang2019improving} & 37.6 \\
                AutoGAN~\cite{gong2019autogan}   & 31.0 \\
                DC-VAE~\cite{dcvae}    & 41.91\\
                \midrule
                \midrule
                \textbf{\shortname (Ours)} & \textbf{14.24} \\
                \bottomrule
                \hline
            \end{tabular}
        }
    \end{minipage}
&
    \begin{minipage}[t]{1.5in}
        \caption{\small Generative performance on ImageNet 32.} 
        \label{tab:imagenet}
        \centering
        \scalebox{0.8}{
            \begin{tabular}{@{}lc@{}}
                \hline
                \toprule
                \textbf{Model} & \textbf{FID$\downarrow$} \\
                \midrule
                ScoreFlow~\cite{song2021maximum} & 14.14 \\
                FlowMatching~\cite{lipman2023flow} & \textbf{5.02} \\
                \midrule
                \midrule
                PixelCNN~\cite{oord2016conditional} &  40.51\\
                \midrule
                CF-EBM~\cite{zhao2021learning} & 26.31 \\ 
                CLEL-Large~\cite{clel} & 15.47 \\
                \midrule
                \textbf{\shortname (Ours)} & \textbf{8.64} \\
                \bottomrule
                \hline
            \end{tabular}
        }
    \end{minipage}
\end{tabular}
\vspace{-4mm}
\end{table}
% \vspace{-4mm}
